Transferable Perturbations of Deep Feature Distributions

Almost all current adversarial attacks of CNN classifiers rely on information derived from the output layer of the network. This work presents a new adversarial attack based on the modeling and exploitation of class-wise and layer-wise deep feature distributions. We achieve state-of-the-art targeted blackbox transfer-based attack results for undefended ImageNet models. Further, we place a priority on explainability and interpretability of the attacking process. Our methodology affords an analysis of how adversarial attacks change the intermediate feature distributions of CNNs, as well as a measure of layer-wise and class-wise feature distributional separability/entanglement. We also conceptualize a transition from task/data-specific to model-specific features within a CNN architecture that directly impacts the transferability of adversarial examples.

==> sections/methodology_KL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Attack methodology}
\vspace{-2mm}
%%%%
%\subsection{Capturing feature distributions.}
% \textbf{Capturing feature distributions.}
We first assume to have a set of training data and a pre-trained model $f$ from the same task as the target blackbox model (i.e. the ImageNet-1k training set and a pre-trained ImageNet model).
We then explicitly model the feature distributions for a set of source/target classes $\mathcal{C}=\{c_1,...,c_K\}$ and a set of layers of interest $\mathcal{L}=\{l_1,...,l_N\}$.
% The first step to attack is the explicit modeling of the feature distributions, as shown in Figure~\ref{fig:da_figure}(top). To start, we identify a set of classes $\mathcal{C}=\{c_1,...,c_K\}$ that we are interested in targeting, and a set of layers $\mathcal{L}=\{l_1,...,l_N\}$ that we are keen to probe.
For each layer in $\mathcal{L}$, we train a small, binary, one-versus-all classifier $g$ for each of the classes in $\mathcal{C}$. Each binary classifier is given a unique set of parameters, and referred to as auxiliary model $g_{l,c}$. Thus, we say that $g_{l,c}(f_l(x))$ outputs $p(y=c|f_l(x))$, where $f_l(x)$ is the layer $l$ feature map of the pre-trained model $f$ given input image $x$.

%%%%
%\subsection{Attack objectives}
% \textbf{Attack objectives.}  
%Unlike many attack formulations that use the logit or output probability information of the whitebox model to craft adversarial noise \cite{Dong2018BoostingAA, Madry2018TowardsDL, Goodfellow2015ExplainingAH, Carlini2016TowardsET}, our methods use the captured feature distributions exclusively. 
Once trained, we may leverage the learned feature distributions to create both targeted and untargeted adversarial examples. Here, we focus mostly on targeted attacks, which are considered a harder problem (especially in the blackbox transfer case when we do not have access to the target model's gradients). Discussion of untargeted attacks is left to Appendix C. Recall, the goal of a targeted attack is to generate an adversarial noise $\delta$ that when added to a clean sample $x$ of class $y_{src}$, the classification result of $x+\delta$ is a chosen class $y_{tgt}$. The key intuition for our targeted attacks is that if a sample has features consistent with the feature distribution of class $c$ at some layer of deep feature space, then it will likely be classified as class $c$. Although not shown in the objective functions for simplicity, for all attacks the adversarial noise $\delta$ is constrained by an $\ell_p$ norm (i.e. $||\delta||_p<\epsilon$), and the choice of layer $l$ and target class label $y_{tgt}$ are chosen prior to optimization. 
We propose three attack variants for generating targeted adversarial examples:

\vspace{-2mm}
\paragraph{\FDA} The most straightforward attack is to find a perturbation $\delta$ of the ``clean'' input image $x$ that maximizes the probability that the layer $l$ features are from the target class $y_{tgt}$ distribution:
\begin{equation}
\max_{{\delta}} p(y=y_{tgt}|f_l(x+\delta)).
\end{equation}
This resembles attack objectives common in the literature, but we stress that we target intermediate feature distributions and not just the logit layer, thus calling it Feature Disruption Attack (\FDA).

\vspace{-2mm}
\paragraph{\FDAms} In addition to the objective of \FDA, we may also choose to minimize the probability that the layer $l$ features are from the source class $y_{src}$ distribution (\textit{ms} = minimize source):
\begin{equation}
\max_{{\delta}} \lambda p(y=y_{tgt}|f_l(x+\delta)) - (1-\lambda) p(y=y_{src}|f_l(x+\delta)).
\end{equation}
where $\lambda$ weights the contribution of both terms and is a fixed, positive value. 

\vspace{-2mm}
\paragraph{\FDAfd} Alternatively, rather than minimizing the source distribution probability, we may instead seek to maximize ``feature disruption'' (\textit{fd}), pushing the layer $l$ features of the perturbed sample to be maximally different from the original sample:
\begin{equation}
\max_{{\delta}} p(y=y_{tgt}|f_l(x+\delta)) + \eta \frac{\left\Vert f_l(x+\delta) - f_l(x) \right\Vert _2}{\left\Vert f_l(x) \right\Vert _2}.
\end{equation}
where $\eta$ is a fixed positive value weight for the feature disruption term. 
% \FDAfd\ maximizes the probability that the layer $l$ features are from the target class distribution while also maximizing the distance of the perturbed features from the original features. 

Notice, the additional terms in \FDAms\ and \FDAfd\ encourage the adversarial sample to move far away from the starting point which may intuitively help in generating (targeted) adversarial examples. Also notice that \FDAms\ requires the modeling of both the source and target class distributions whereas the others only require the modeling of the target class distribution. 

\textbf{Optimization Procedure.}
The trained auxiliary models afford a way to construct a fully differentiable path for gradient-based optimization of the objective functions. Specifically, to compute \FDA\ adversarial noise from layer $l$, we first build a composite model using the truncated whitebox model $f_l$ and the corresponding layer's auxiliary model $g_{l,c=y_{tgt}}$ for the target class $y_{tgt}$, as shown in Figure~\ref{fig:da_figure}(bottom). The loss is calculated as the Binary Cross Entropy (BCELoss) between the predicted $p(y=y_{tgt}|f_l(x))$ and 1. Thus, we perturb the input image in the direction that will minimize the loss, in turn maximizing $p(y=y_{tgt}|f_l(x)$. For optimization, we employ iterative gradient descent with momentum, as the inclusion of a momentum term in adversarial attacks has proven effective \citep{Inkawhich_2019_CVPR,Dong2018BoostingAA}. See Appendix D for more details.
